On the Diachronic Stability of Irregularity in Inflectional Morphology

Many languages' inflectional morphological systems are replete with irregulars, i.e., words that do not seem to follow standard inflectional rules. In this work, we quantitatively investigate the conditions under which irregulars can survive in a language over the course of time. Using recurrent neural networks to simulate language learners, we test the diachronic relation between frequency of words and their irregularity.

==> table2.tex <==
\begin{figure*}
\begin{adjustbox}{width=2\columnwidth}
 \begin{tikzpicture}
   \begin{axis}[
       axis x line*=bottom, axis y line*=left,
       ybar=0pt,
       ymin=0,
               xlabel={Generation 1},
       ylabel={$D_{\textit{KL}}$},
       y label style={at={(axis description cs:-0.1,0.5)}},
        % xlabel={Generation 1},
        % x label style={at={(axis description cs:0.5,-0.1)}},
        bar width=7pt,
        ymajorgrids,
        yminorgrids,
        symbolic x coords={unigram,uniform,class},
       enlarge x limits={value=0.25, auto},
       xtick=data,
       nodes near coords align={horizontal}, every node near coord/.append style={rotate=90},
       width=16em, height=14em,
       legend style={at={(1.1,0.5)},anchor=west,draw=none,fill=none,column sep=1em,name=legend},
       legend columns=1,
       legend cell align=left
       ]
     \addplot[  red!50!black,fill=  red!50!white] coordinates {(unigram, 1.13) (uniform, 30.63) (class, 40.83)};
     \addplot[ blue!35!black,fill= blue!35!white] coordinates {(unigram, 1.13) (uniform, 30.63) (class, 40.83)};
     \addplot[green!35!black,fill=green!35!white] coordinates {(unigram, 1.49) (uniform, 0.41) (class, 0.54)};
     \addplot[brown!65!black,fill=brown!65!white] coordinates {(unigram, 11.34) (uniform, 424.21) (class, 616.61)};
      % \legend{all,all$_{\textit{gold}}$,reg$_{\textit{gold}}$,irreg$_{\textit{gold}}$}
    \end{axis}
 \end{tikzpicture}
\begin{tikzpicture}
   \begin{axis}[
        axis x line*=bottom, axis y line*=left,
        ybar=0pt,
        ymin=0,
                xlabel={Generation 2},
        % ylabel={0/1},
        % y label style={at={(axis description cs:-0.1,0.5)}},
        % xlabel={Generation 2},
        % x label style={at={(axis description cs:0.5,-0.1)}},
        bar width=7pt,
        ymajorgrids,
        yminorgrids,
        symbolic x coords={unigram,uniform,class},
       enlarge x limits={value=0.25, auto},
       xtick=data,
       nodes near coords align={horizontal}, every node near coord/.append style={rotate=90},
       width=16em, height=14em,
       legend style={at={(1.1,0.5)},anchor=west,draw=none,fill=none,column sep=1em,name=legend},
       legend columns=1,
       legend cell align=left
       ]
     \addplot[  red!50!black,fill=  red!50!white] coordinates {(unigram, 0.32) (uniform, 0.23) (class, 0.53)};
     \addplot[ blue!35!black,fill= blue!35!white] coordinates {(unigram, 8.72) (uniform, 239.17) (class, 78.54)};
     \addplot[green!35!black,fill=green!35!white] coordinates {(unigram, 8.16) (uniform, 8.79) (class, 4.84)};
     \addplot[brown!65!black,fill=brown!65!white] coordinates {(unigram, 107.29) (uniform, 4288.35) (class, 1357.41)};
      % \legend{all,all$_{\textit{gold}}$,reg$_{\textit{gold}}$,irreg$_{\textit{gold}}$}
    \end{axis}
 \end{tikzpicture}
  %
  \begin{tikzpicture}
   \begin{axis}[
        axis x line*=bottom, axis y line*=left,
        ybar=0pt,
        ymin=0,
                xlabel={Generation 2},
        % ylabel={0/1},
        % y label style={at={(axis description cs:-0.1,0.5)}},
        % xlabel={Generation 3},
        % x label style={at={(axis description cs:0.5,-0.1)}},
        bar width=7pt,
        ymajorgrids,
        yminorgrids,
        symbolic x coords={unigram,uniform,class},
       enlarge x limits={value=0.25, auto},
       xtick=data,
       nodes near coords align={horizontal}, every node near coord/.append style={rotate=90},
       width=16em, height=14em,
       legend style={at={(1.1,0.5)},anchor=west,draw=none,fill=none,column sep=1em,name=legend},
       legend columns=1,
       legend cell align=left
       ]
     \addplot[  red!50!black,fill=  red!50!white] coordinates {(unigram, 0.34) (uniform, 0.24) (class, 0.32)};
     \addplot[ blue!35!black,fill= blue!35!white] coordinates {(unigram, 11.92) (uniform, 254.27) (class, -85.43)};
     \addplot[green!35!black,fill=green!35!white] coordinates {(unigram, 11.34) (uniform, 14.74) (class, 6.78)};
     \addplot[brown!65!black,fill=brown!65!white] coordinates {(unigram, 129.72) (uniform, 4503.88) (class, 1478.45)};
     \legend{all,all$_{\textit{gold}}$,reg$_{\textit{gold}}$,irreg$_{\textit{gold}}$}
   \end{axis}
 \end{tikzpicture}
\end{adjustbox}
\caption{Here, we have the same breakdown as in \cref{fig:accuracy}, but, instead of accuracy, we report the $D_\textit{KL}$. }
\end{figure*}
